Doubling the order of approximation via the randomized product formula

Randomization has been applied to Hamiltonian simulation in a number of ways to improve the accuracy or efficiency of product formulas. Deterministic product formulas are often constructed in a symmetric way to provide accuracy of even order 2k. We show that by applying randomized corrections, it is possible to more than double the order to 4k + 1 (corresponding to a doubling of the order of the error). In practice, applying the corrections in a quantum algorithm requires some structure to the Hamiltonian, for example the Pauli strings as are used in the simulation of quantum chemistry.

==> removed.tex <==
%Then we use the Neumann series to have
%\begin{align}
%        &\sum_{l \in \gamma}\sum_{h=1}^{L_{l}}p_{h,l}S_{2k}U_{h}^{(l)}S_{2k}\nn
%        &=S_{2k}(I+V^{\dagger}D)^{-1}(I+DV^{\dagger})^{-1}S_{2k} + S_{2k}\biggl(\sum_{l\in \gamma}\sum_{h=1}^{L_{l}} \frac {|\epsilon_{h,l}|}{A}\sum_{i=2}^{\infty}\frac{1}{i!}(\alpha_{h,l} H_{h}^{(l)})^{i}\biggr)S_{2k}\nn
%        & \quad \quad + S_{2k}[R_{4k+1}(V^{\dagger}D+DV^{\dagger})]S_{2k}- S_{2k}V^{\dagger}D DV^{\dagger}S_{2k}\nn
%        & \quad \quad + S_{2k}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(V^{\dagger} D)^{i}\biggr](I+DV^{\dagger})^{-1}S_{2k}\nn 
%        & \quad \quad+S_{2k}(I+V^{\dagger}D)^{-1}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]S_{2k}.
%\end{align}

\begin{comment}
Next, note that $A$ corresponds to the sum of the magnitudes of the terms in $V^\dagger D+DV^\dagger$, where both quantities are on $\lambda/2$.
In order to bound the sum of the magnitudes of terms here, note the upper bound on the order-$s$ error in Eq.~(49) of \cite{childs2019faster} is given as
\begin{equation}
    \frac{2(2L 5^{k-1}|\lambda| \Lambda)^s}{s!}
\end{equation}
for interval $\lambda$ (we will replace it with $\lambda/2$ for $D$ below).
That expression is in turn based on the bound used in Eq.~(8) of \cite{berry2007efficient}.
That expression is using $2(L-1)5^{k-1}+1$ for the number of exponentials in the product for $S_{2k}$, but for simplicity it can be replaced with the upper bound $2L5^{k-1}$.
That would give an upper bound of $(2L 5^{k-1}|\lambda| \Lambda)^s/s!$ for the order $s$ terms in the expansion of $S_{2k}$, and in Eq.~(49) of \cite{childs2019faster} it is simply multiplied by 2.

Using the approach in \cite{berry2007efficient}, one would instead add the order-$s$ terms from the exact exponential, which can be upper bounded by $(L |\lambda| \Lambda)^s/s!$.
That gives a replacement of the upper bound from \cite{childs2019faster} with
\begin{equation}\label{eq:orderserror}
    \frac{[1+(2\times 5^{k-1})^s](L|\lambda| \Lambda)^s}{s!}.
\end{equation}
That can be summed to give the upper bound on the error, and here we will need to replace $\lambda$ with $\lambda/2$.
In contrast, if we were to multiply $S_{2k}$ by the inverse of the evolution, one can use the same approach as in \cite{berry2007efficient} and replace the power with $2L5^{k-1}+L$ (with the $+L$ coming from the inverse evolution).
Then one can give the upper bound on the order-$s$ term as
\begin{equation}\label{eq:orderserrorVD}
    \frac{(1+2\times 5^{k-1})^s(L|\lambda| \Lambda)^s}{s!}.
\end{equation}
You can see that the difference here is the $1+$ now appears inside the brackets.
\end{comment}

\begin{comment}
{\color{red} This part does not look right.
where we use Lemma \ref{V_D} in the last equality.
Now we have
\begin{align}
     \biggl\|S_{2k}[R_{4k+1}(V^{\dagger}D+DV^{\dagger})]S_{2k} \biggr\|
     &\leq  8\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\sum_{i=2k+1}^{\infty}\frac{([\kappa+1]|\lambda|L\Lambda/2))^{i}}{i!}\nn
     &\leq  8\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\frac{([\kappa+1]|\lambda|L\Lambda/2))^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2))\nn
     &=8\frac{([\kappa(\kappa+1)]^{2k+1}(|\lambda|L\Lambda/2)^{4k+2}}{((2k+1)!)^{2}}\exp([\kappa+1]|\lambda|L\Lambda/2)).
\end{align}}
\end{comment}

\begin{comment}
In order to bound the sum of the magnitudes of terms here, note the upper bound on the order-$s$ error in Eq.~(49) of \cite{childs2019faster} is given as
\begin{equation}
    \frac{2(2L 5^{k-1}|\lambda| \Lambda)^s}{s!}
\end{equation}
for interval $\lambda$ (we will replace it with $\lambda/2$ for $D$ below).
That expression is in turn based on the bound used in Eq.~(8) of \cite{berry2007efficient}.
That expression is using $2(L-1)5^{k-1}+1$ for the number of exponentials in the product for $S_{2k}$, but for simplicity it can be replaced with the upper bound $2L5^{k-1}$.
That would give an upper bound of $(2L 5^{k-1}|\lambda| \Lambda)^s/s!$ for the order $s$ terms in the expansion of $S_{2k}$, and in Eq.~(49) of \cite{childs2019faster} it is simply multiplied by 2.
\end{comment}

\begin{comment}
Next, for the second norm in Eq.~(\ref{VS_2}), we use the submultiplicative property of the spectral norm and Lemma \ref{V_D} to have 
\begin{align}
    \biggl\| S_{2k}V^{\dagger}D DV^{\dagger}S_{2k} \biggr\| 
    \leq  \|V^{\dagger}D DV^{\dagger}\|
    &\leq (\|V^{\dagger}\|\cdot \|D\|)^{2}\nn
    & \leq \biggl(2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2)  \biggr)^{2}\nn
    &=4\frac{(\kappa|\lambda|L\Lambda/2)^{4k+2}}{((2k+1)!)^{2}}\exp(2[\kappa+1]|\lambda|L\Lambda/2).
\end{align}
Finally, for the norms in Eq.~(\ref{VS_3}), we use the the submultiplicative property of the spectral norm to have
\begin{align}
\biggl\|S_{2k}(I+V^{\dagger}D)^{-1}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]S_{2k} \biggr\| 
&\leq  \|S_{2k}\|\cdot \biggl\|(I+V^{\dagger}D)^{-1}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]\biggr\| \cdot\|S_{2k} \| \nn
&\leq \biggl\|(I+V^{\dagger}D)^{-1}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]\biggr\|. 
\end{align}
Next, we use the Newmann series and some basic norm properties to obtain
\begin{align}
    \biggl\|S_{2k}(I+V^{\dagger}D)^{-1}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]S_{2k} \biggr\|
    &\leq \biggl\|\biggl[\sum_{n=0}^{\infty}(-1)^{i}(V^{\dagger}D)^{i}\biggr]\biggl[\sum_{i=2}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]\biggr\| \nn
    &\leq \biggl[\sum_{n=0}^{\infty}(\|V^{\dagger}\|\cdot \|D\|)^{i}\biggr]\biggl[\sum_{i=2}^{\infty}(\|D\|\cdot \|V^{\dagger}\|)^{i}\biggr]\biggr\| \nn
    &=\frac{(\|V^{\dagger}\|\cdot \|D\|)^{2}}{(1-\|V^{\dagger}\|\cdot \|D\|)^{2}}.
\end{align}
Similarly, we can have the same bound for the norm
\begin{align}
     \biggl \|S_{2k}\biggl[\sum_{i=2}^{\infty}(-1)^{i}(V^{\dagger} D)^{i}\biggr](I+DV^{\dagger})^{-1}S_{2k}\biggr\|
     &\leq \biggl\|\biggl[\sum_{i=2}^{\infty}(-1)^{i}(V^{\dagger}D)^{i}\biggr]\biggl[\sum_{n=0}^{\infty}(-1)^{i}(DV^{\dagger})^{i}\biggr]\biggr\| \nn
     &\leq \biggl[\sum_{i=2}^{\infty}(\|V^{\dagger}\|\cdot \|D\|)^{i}\biggr]\biggl[\sum_{n=0}^{\infty}(\|D\|\cdot \|V^{\dagger}\|)^{i}\biggr]\biggr\| \nn
     &=\frac{(\|V^{\dagger}\|\cdot \|D\|)^{2}}{(1-\|V^{\dagger}\|\cdot \|D\|)^{2}},
\end{align}
where we have $\|V^{\dagger}\|\cdot \|D\| \leq 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2)$ from Lemma \ref{V_D}.
\end{comment}

%This indicates that we can design a set of unitary $\{U_{h}^{(l)}\}$
%\begin{equation}
%U_{h}^{(l)}:=\exp\biggl(\lambda^{l}\alpha_{h,l}H_{h}^{(l)}\biggr),
%\end{equation}
%and the corresponding probabilities $\{p_{h,l}\}$ such that 
%\begin{align}
%    V^{\dagger} \sum_{l \in \gamma}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
%        U_{h}^{(l)}=I+O(\lambda^{4k+2})
%\end{align}
%
%
%From Eq.~(\ref{eq_error_2k+1}), we have the bound after some modifications
%\begin{equation}
%  \biggl\Vert I-V(-\lambda) S_{p}^{(2k)}(\lambda) \biggr\Vert \leq \frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L).
%\end{equation}


\begin{comment}
Next, we rewrite it as
\begin{align}
     &\sum_{l \in \gamma}\sum_{h=1}^{L_{l}}p_{h,l}S^{(2k)}U_{h}^{(l)}S^{(2k)} \nn
     &=S^{(2k)}\biggl(I-\sum_{l\in \gamma'}\sum_{h=1}^{L_{l}}\biggl(\frac{\lambda}{2}\biggr)^{l}\beta_{h}^{(l)} V^{\dagger}H_{h}^{(l)}\biggl)\biggr(I- \sum_{l \in \gamma'}\sum_{h=1}^{L_{l}}\biggl(\frac{\lambda}{2}\biggr)^{l}\beta_{h}^{(l)}H_{h}^{(l)} V^{\dagger}\biggr) S^{(2k)}+O(\lambda^{4k+2}),
\end{align}
where $\gamma'=\{2k+2n-1: n\in \mathbb{N}\}$.
Then we use the Neumann series to have
\begin{align}
        &\sum_{l \in \gamma}\sum_{h=1}^{L_{l}}p_{h,l}S^{(2k)}U_{h}^{(l)}S^{(2k)} \nn
        &=  S^{(2k)}\biggl(I+\sum_{l \in \gamma'}\sum_{h=1}^{L_{l}}\biggl(\frac{\lambda}{2}\biggr)^{l}\beta_{h}^{(l)} V^{\dagger}H_{h}^{(l)}\biggl)^{-1}\biggr(I+ \sum_{l \in \gamma'}\sum_{h=1}^{L_{l}}\biggl(\frac{\lambda}{2}\biggr)^{l}\beta_{h}^{(l)}H_{h}^{(l)} V^{\dagger}\biggr)^{-1} S^{(2k)} +O(\lambda^{4k+2}).
\end{align}
Notice that 
\begin{align}
    \sum_{l \in \gamma'}\sum_{h=1}^{L_{l}}\biggl(\frac{\lambda}{2}\biggr)^{l}\beta_{h}^{(l)}\cdot V^{\dagger}(\lambda/2)\cdot H_{h}^{(l)}=V^{\dagger}(\lambda/2)\cdot S^{(2k)}(\lambda/2)-I.
\end{align}
Ultimately, we can construct the modified randomized formula with the $(4k+1)$th-order approximation 
\begin{equation}
    \begin{split}
S^{(4k+1)}(\lambda):=\sum_{l \in \gamma}\sum_{h=1}^{L_{l}} p_{h,l} S^{(2k)}(\lambda/2)U_{h}^{(l)}S^{(2k)}(\lambda/2 ).
    \end{split}
\end{equation}
\end{comment}

       % &=  S^{(2k)}\biggl(I+ \sum_{l \in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\alpha_{h,l} H_{h}^{(l)}\biggr) S^{(2k)}+O(\lambda^{4k+2}) \nn
%        &=  S^{(2k)}\biggl(\openone-V^{\dagger}D \biggr)\biggl(I-DV^{\dagger}\biggr) S^{(2k)} +O(\lambda^{4k+2})\nn
%        &=  S^{(2k)}\biggl(\openone+V^{\dagger}D \biggr)^{-1}\biggl(I+DV^{\dagger}\biggr)^{-1} S^{(2k)} +O(\lambda^{4k+2}) \label{VD-1}\\
%        &=  S^{(2k)}\biggl(V^{\dagger}S^{(2k)}\biggl)^{-1}\biggr(S^{(2k)}V^{\dagger}\biggr)^{-1} S^{(2k)}+O(\lambda^{4k+2}) \nn

\begin{comment}
where $\{\beta_{i}^{(l)'}\}$ is defined from
\begin{equation} \label{H'}
V^{\dagger} S_{p}^{(2k)}:=I+\sum_{l=2k+1}^{\infty} \lambda^{l} \mathcal{H}_{l}',
\end{equation}
where
\begin{equation}
\mathcal{H}_{l}':=\sum_{i=1}^{L_{l}}\beta_{i}^{(l)'}H_{i}^{(l)}.
\end{equation}
\end{comment}

\begin{comment}
If we can design a set of unitaries $\{U_{h}^{(2k)}\}$, where $h \in \{1,2,...,L_{2k+1}\}$ 
\begin{equation}\label{U_{h}^{(2k)}}
U_{h}^{(2k)}:=\exp\biggl(\lambda^{2k+1}\alpha_{h}H_{h}^{(2k+1)}\biggr),
\end{equation}
with some probability $\{p_{h} \}$ and designed coefficients $\{\alpha_{h}\}$
so that the average over the term \\$ S_{p}^{(2k)}\cdot U_{h}^{(2k)}$ satisfies 
\begin{equation} \label{1/n_S_{p}^{(2k)}}
\begin{split}
        &\sum_{h=1}^{L_{2k+1}}p_{h}S_{p}^{(2k)}
        \cdot U_{h}^{(2k)} \\
        &=I + \sum_{l=1}^{2k}\lambda^{l} \mathcal{H}_{l} +\frac{\lambda^{2k+1}}{(2k+1)!}\cdot \sum_{i=1}^{L_{2k+1}}H_{i}^{(2k+1)}+O(\lambda^{2k+2}),
\end{split}
\end{equation}
the modified product formula in Eq.~\eqref{1/n_S_{p}^{(2k)}} could yield the approximation error to order $O(|\lambda|^{2k+2})$.
Consequently, the condition in Eq.~\eqref{1/n_S_{p}^{(2k)}} leads to the constraint for the coefficient $\{\alpha_{h}\}$ and probabilities $\{p_{h}\}$ given below
\begin{equation}\label{alpha_beta_11}
p_{h}\alpha_{h}= \frac 1{(2k+1)!} - \beta_{h}^{(2k+1)}.
\end{equation}
%{\color{red}Why is there division by $\Vert H_{h}^{(2k+1)}\Vert$ here?}
From the criterion in Eq.~\eqref{alpha_beta_11}, we could choose 
\begin{align}
    p_h &:= \frac {|\epsilon_{h}^{(2k+1)}|}{A_{2k+1}},\\
    \alpha_{h} &:= \frac{{\rm sign}(\epsilon_{h}^{(2k+1)})A_{2k+1}}{\|H_{h}^{(2k+1)}\|},
\end{align}
where
\begin{align}
    \epsilon_{h}^{(2k+1)} &:= \left(\frac 1{(2k+1)!} - \beta_{h}^{(2k+1)}\right) \|H_{h}^{(2k+1)}\|, \\
     A_{2k+1} &:= \sum_{h=1}^{L_{2k+1}} |\epsilon_{h}^{(2k+1)}|.
\end{align}
The choice of criterion in Eq.~(\ref{alpha_beta_11}) can be easily derived by the following simple calculation 
\begin{align}
        \sum_{h=1}^{L_{2k+1}} p_h S_{p}^{(2k)}
        \cdot U_{h}^{(2k)}
        &=\sum_{h=1}^{L_{2k+1}}\frac {|\epsilon_{h}^{(2k+1)}|}{A_{2k+1}}\biggl(I+ \sum_{l=1}^{\infty} \lambda^{l} \mathcal{H}_{l}\biggr)\biggl(1+ \lambda^{2k+1}\alpha_{h} H_{h}^{(2k+1)}+ O(\lambda^{4k+2})\biggr)\nn
        &=\biggl(I+ \sum_{l=1}^{\infty} \lambda^{l} \mathcal{H}_{l}\biggr)\biggl(1+ \lambda^{2k+1}\sum_{h=1}^{L_{2k+1}}\frac {|\epsilon_{h}^{(2k+1)}|}{A_{2k+1}}\alpha_{h} H_{h}^{(2k+1)}+O(\lambda^{4k+2})\biggr)\nn
        &=I + \sum_{l=1}^{2k} \lambda^{l} \mathcal{H}_{l}+ \lambda^{2k+1} \mathcal{H}_{2k+1} +\lambda^{2k+1}\sum_{h=1}^{L_{2k+1}}\frac {|\epsilon_{h}^{(2k+1)}|}{A_{2k+1}}\alpha_{h} H_{h}^{(2k+1)}+O(\lambda^{2k+2})\nn
        %
%        &=I + \sum_{l=1}^{2k} \lambda^{l} \mathcal{H}_{l} + \lambda^{2k+1} \sum_{h=1}^{L_{2k+1}} \beta_i^{(2k+1)} H_{h}^{(2k+1)}
%        + \lambda^{2k+1} \sum_{h=1}^{L_{2k+1}} \left(\frac 1{(2k+1)!} - \beta_i^{(2k+1)}\right) H_{h}^{(2k+1)}+O(\lambda^{2k+2}) \\
        &=I + \sum_{l=1}^{2k} \lambda^{l} \mathcal{H}_{l} +  \sum_{h=1}^{L_{2k+1}} \frac {\lambda^{2k+1}}{(2k+1)!} H_{h}^{(2k+1)}+O(\lambda^{2k+2}).
\end{align}
\end{comment}

\begin{comment}
\begin{align}\label{Sp2k_&_ph}
        \sum_{h=1}^{L_{2k+1}}&p_{h}S_{p}^{(2k)}
        \cdot U_{h}^{(2k)}\\
        &=\sum_{h\in \eta^{(2k+1)}}p_{h}\biggl(1+ \sum_{l=1}^{\infty} \lambda^{l} \mathcal{H}_{l}\biggr)\biggl(1+ \lambda^{2k+1}\alpha_{h}H_{h}^{(2k+1)}+O(\lambda^{4k+2})\biggr)\\
        &=I + \sum_{l=1}^{2k} \lambda^{l} \mathcal{H}_{l} + \lambda^{2k+1} \sum_{s\in \gamma^{(2k+1)}} \sum_{j\in \{1,2,...,m_{s}^{(2k+1)}\}}\biggl(\frac{\alpha_{(s,j)}}{n}+\beta_{s}^{(2k+1)}\biggr)H_{s}^{(2k+1)}\\
        &\quad \quad +\frac{\lambda^{2k+1}}{(2k+1)!} \sum_{i\in \gamma^{(2k+1)'}}H_{i}^{(2k+1)}+O(\lambda^{2k+2}),
\end{align}
and the above calculations also hold for the case of the average over $U_{h}^{(2k)} \cdot S_{p}^{(2k)}$.

{\color{blue}Dominic:  Here is a better way of doing it.\\
Let us define
\begin{align}
    \epsilon_{i} &:= \left(\frac 1{(2k+1)!} - \beta_i^{(2k+1)}\right) \|H_{i}^{(2k+1)}\|, \\
    A_{2k+1} &:= \sum_i |\epsilon_{i}^{(2k+1)}|, \\
    \alpha_{i} &:= \frac{{\rm sign}(\epsilon_{i})A_{2k+1}}{\|H_{i}^{(2k+1)}\|}
\end{align}
Then choose unitary
\begin{equation}
U_{h}^{(2k)}:=\exp\biggl(\lambda^{2k+1}\alpha_{h}H_{h}^{(2k+1)}\biggr),
\end{equation}
with probability
\begin{equation}
    p_h = \frac {|\epsilon_{h}|}{A_{2k+1}}.
\end{equation}
You then find that
\begin{align}
        &\sum_{h} p_h S_{p}^{(2k)}
        \cdot U_{h}^{(2k)}\\
        &=\sum_{h}\frac {|\epsilon_{h}|}{A_{2k+1}}\biggl(I+ \sum_{l=1}^{\infty} \lambda^{l} \mathcal{H}_{l}\biggr)\biggl(1+ \lambda^{2k+1}\alpha_{h} H_{h}^{(2k+1)}+O(\lambda^{4k+2})\biggr)\\
        &=I + \sum_{l=1}^{\infty} \lambda^{l} \mathcal{H}_{l} + \lambda^{2k+1} \sum_{h} \frac {|\epsilon_{h}|}{A_{2k+1}} {\rm sign}(\epsilon_{h}) A_{2k+1} H_{h}^{(2k+1)}/\|H_{h}^{(2k+1)}\|+O(\lambda^{2k+2})\\
        &=I + \sum_{l=1}^{\infty} \lambda^{l} \mathcal{H}_{l} + \lambda^{2k+1} \sum_{h} \epsilon_{h} H_{h}^{(2k+1)}/\|H_{h}^{(2k+1)}\|+O(\lambda^{2k+2})\\
        &=I + \sum_{l=1}^{2k} \lambda^{l} \mathcal{H}_{l} + \lambda^{2k+1} \sum_{h} \beta_i^{(2k+1)} H_{h}^{(2k+1)}
        + \lambda^{2k+1} \sum_{h} \left(\frac 1{(2k+1)!} - \beta_i^{(2k+1)}\right) H_{h}^{(2k+1)}+O(\lambda^{2k+2}) \\
        &=I + \sum_{l=1}^{2k} \lambda^{l} \mathcal{H}_{l} +  \sum_{h} \frac {\lambda^{2k+1}}{(2k+1)!} H_{h}^{(2k+1)}+O(\lambda^{2k+2})
\end{align}
To explain the higher-order corrections, for imaginary $\lambda$ we can say that
\begin{equation}
  \biggl\Vert I-V(-\lambda) S_{p}^{(2k)}(\lambda) \biggr\Vert \leq \frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L).
\end{equation}
We can therefore write
\begin{equation}
V(-\lambda) S_{p}^{(2k)}=I+\sum_{l=2k+1}^{\infty} \lambda^{l} \mathcal{H}_{l},
\end{equation}
with\begin{equation}
\mathcal{H}_{l}:=\sum_{i=1}^{L_{l}}\beta_{i}^{(l)}H_{i}^{(l)}.
\end{equation}
In this description the quantities $\beta_{i}^{(l)}$ are different from the previous version.
Now we define
\begin{align}
    \epsilon_{i,l} &:= \lambda^l\beta_i^{(l)}  \|H_{i}^{(l)}\|, \\
    A &:= \sum_{l=2k+1}^{4k+2}\sum_{i=1}^{L_{l}} |\epsilon_{i,l}|, \\
    \alpha_{i,l} &:= -\frac{{\rm sign}(\epsilon_{i,l})A}{\|H_{i}^{(l)}\|}
\end{align}
The bound on the error means that
\begin{equation}
    A \le \frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L).
\end{equation}
Then choose unitary
\begin{equation}
U_{h}^{(l)}:=\exp\biggl(\alpha_{h,l}H_{h}^{(l)}\biggr),
\end{equation}
with probability
\begin{equation}
    p_{h,l} = \frac {|\epsilon_{h,l}|}{A}.
\end{equation}
You then find that
\begin{align}
        &V(-\lambda) \sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
        \cdot U_{h}^{(l)}\\
        &=  \sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\biggl(I+ \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}\biggr)\biggl(I+ \alpha_{h,l} H_{h}^{(l)}+(\alpha_{h,l} H_{h}^{(l)})^2+O(\lambda^{6k+3})\biggr)\\
        &=  \biggl(I+ \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}\biggr)\biggl(I- 
        \sum_{l=2k+1}^{4k+2} \lambda^{l} \mathcal{H}_{l}
        +\sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} \frac {|\epsilon_{h,l}|}{A}(\alpha_{h,l} H_{h}^{(l)})^2+O(\lambda^{6k+3})\biggr)\\
        &= I + \sum_{l=4k+3}^{\infty} \lambda^{l} \mathcal{H}_{l} - \left( \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell} \right) \left(  \sum_{l=2k+1}^{4k+2} \lambda^{l} \mathcal{H}_{l}\right) \\
        & \quad -\sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} \lambda^l\beta_i^{(l)} \alpha_{h,l} (H_{h}^{(l)})^2+O(\lambda^{6k+3})
\end{align}
Now
\begin{equation}
    \left\| \left( \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell} \right) \left(  \sum_{l=2k+1}^{4k+2} \lambda^{l} \mathcal{H}_{l}\right)\right\| \le \left[\frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L)\right]^2
\end{equation}
and
\begin{align}
\left\|\sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} \lambda^l\beta_i^{(l)} \alpha_{h,l} (H_{h}^{(l)})^2\right\| &\le
\sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} \lambda^l|\beta_i^{(l)}| \times \| H_{h}^{(l)}\| A \le A^2 .
\end{align}
As a result we have
\begin{equation}
    \left\| I - V(-\lambda) \sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
        \cdot U_{h}^{(l)}\right\| \le 2\left[\frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L)\right]^2
        + O(\lambda^{4k+3}).
\end{equation}
In turn that implies
\begin{equation}
    \left\| V(\lambda) - \sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
        \cdot U_{h}^{(l)}\right\| \le 2\left[\frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L)\right]^2
        + O(\lambda^{4k+3}).
\end{equation}
Here we have limited the corrections to order $\lambda^{4k+2}$ to reduce the number of terms that need to be computed for the correction.
If we were to extend this to higher order, then it would extend the $O(\lambda^{4k+3})$ term on the error bound to higher order, but would not affect the leading-order term in the error.
}
\end{comment}
\begin{comment}
Up to now, we have obtained the recipe for the formula with the $(2k+1)$th-order approximation, and what remains is to further generate the formula with the $(2k+2)$th-order approximation.
This can be achieved with the aid of the results in Lemma \ref{2k+q order error} below, and we leave the proof of Lemma \ref{2k+q order error} in Section \ref{proof_of_lemma}.
\end{comment}
\begin{comment}
Up to now, we have obtained the recipe for the formula with the $(2k+1)$th-order approximation, and what remains is to further generate the formula with the $(4k+1)$th-order approximation.
This can be achieved with the aid of the results in Lemma \ref{2k+q order error} below, and we leave the proof of Lemma \ref{2k+q order error} to Section \ref{proof_of_lemma}.
{\color{red}Is this because we could only guarantee odd-order terms being Hermitian?}
{\color{blue}\begin{lemma} \label{2k+q order error}
%Let $V:=\exp(\lambda\sum_{i=1}^{L} H_i)$, where $\lambda \in \mathbb{C}$ and $|\lambda|\leq 1$
Let $W$ be the target symmetric unitary, and $\{U_h \}$ be a set of unitaries  
which are implemented with the corresponding probabilities $\{p_h \}$. We define
\begin{equation}
    \delta_h := U_h - W,
\end{equation}
and let $\delta_h$ be $O(\lambda^{2k+1})$ for $k \in \mathbb{N}$. We require the conditions that for even $q\le 2k$,
\begin{enumerate}
\item[1.] the $(2k+q-1)$th-order terms in the expansion of $\sum_{h}p_{h}\delta_h$ are cancelled out and 
\item[2.] the $(2k+q)$th-order terms in the expansion of $\sum_{h}p_{h}U_{h}$ are all Hermitian. 
\end{enumerate}
%Then we can deduce that $\sum_{h}p_{h}\delta_h$ is $O(\lambda^{4k})$. 
Then we can deduce that the $(2k+q)$th-order terms in the expansion of $\sum_{h}p_{h}\delta_h$ vanish simultaneously as well.
This guarantees that we can find a way to obtain $\sum_{h}p_{h}\delta_h=O(\lambda^{4k+2})$.
\end{lemma}}
\end{comment}
%{\color{red}The wording here needs to be improved.  The sentence starting ``Provided'' is giving a list of conditions, but a literal interpretation of the way it is worded would be that the later conditions can be inferred from the first condition given.  It would be better to start it with something like ``We require the conditions that''.
%The below part is how to get directly to $4k$ order.}
%Considering the distance between $V$ and $S_{p}^{(2k)}$ \cite{childs2019faster}
%\begin{equation}
%  \biggl\Vert V(\lambda)- S_{p}^{(2k)}(\lambda) \biggr\Vert \leq \frac{(\kappa \Lambda |\lambda|)^{2k+1}L^{2k}}{(2k-1)!}\exp(\kappa \Lambda |\lambda|L),
%\end{equation}


\begin{comment}
\begin{definition} \label{h_v}
 Consider one of the unitary in $\{U_{i}\}_{i=1}^{N_{q}L!}$ as
 \begin{equation}
 \begin{split}
     &S_{2k}^{\sigma}\cdot \exp\biggl( \lambda^{2k+1}\alphaTwo \HTwo\biggr) \cdot \exp\biggl( \lambda^{2k+3}\alphaFour \HFour \biggl)
    \cdots \exp\biggl( \lambda^{2k+q-1}\alphaQ \HQ \biggl),
\end{split}
 \end{equation}
 we can redefine two set of Hamiltonian $\{H_{v}'\}$ and $\{H_{(h_{2v'},v')}'\}$ as the following. 
 The elements in $\{H_{v}'\}_{v=1}^{N}$ are defined as the corresponding Hamiltonian of each exponential term in $S_{2k}^{\sigma}$, and the elements in $\{ H_{(h_{2v'},v')}'\}_{v'=1}^{q/2}$ are defined as
 \begin{equation}
     \begin{split}
         &H_{(h_{2},1)}':= \alphaTwo \HTwo\\
         &H_{(h_{4},2)}':= \alphaFour \HFour\\
         &\quad \quad \quad\vdots \\
         &H_{(h_{q},\frac{q}{2})}':= \alphaQ \HQ.
     \end{split}
 \end{equation}
\end{definition}
\end{comment}
%where we define $\frac{1}{N_{q}}=\frac{1}{2^{q/2}n_{2}n_{4}\cdots n_{q}}$ for simplicity.

\begin{comment}
We define $D$ explicitly as
\begin{align}
    D:=\sum_{l=2k+1}^{\infty} \lambda^{l} \mathcal{H}_{l},
\end{align}
where $\mathcal{H}_{l}$ is defined as the linear combination of the $L_{l}$ elements in the set $\{H_{i}^{(l)}\}_{i=1}^{L_{l}}$, which is composed of the products of $l$ individual Hamiltonian from $\{H_i\}_{i=1}^L$.
%{\color{red}At this point we need the condition that the product is also Hermitian so we can have evolution under it.}
Specifically, we could enumerate all the distinct terms in $\mathcal{H}_{l}$ so that 
\begin{equation}
\mathcal{H}_{l}:=\sum_{i=1}^{L_{l}}\beta_{i}^{(l)}H_{i}^{(l)},
\end{equation}
where $\{\beta_{i}^{(l)}\}_{i=1}^{L_{l}}$ is the coefficient of the term $H_{i}^{(l)}$ in $\mathcal{H}_{l}$. 
\end{comment}


\section{Appendix} \label{appendix}
\subsection{For the case of Trotter-Suzuki formula}
\begin{lemma} \label{V_D}
When we consider the $(2k)$th-order Trotter-Suzuki formula in Eq.~(\ref{S_V_D}), we have the bound
\begin{align}
    \| V^{\dagger}(\lambda/2) \| \|D(\lambda/2)\| \leq 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
\end{align}
\end{lemma}
\begin{proof}
     If we consider $S^{(2k)}(\lambda/2)$ as the $(2k)$th-order Trotter-Suzuki formula, we have
    \begin{align}
        \|D\|
        &=\biggl\| R_{2k}\biggl(\exp(\lambda \sum_{i=1}^{L}H_{i}/2)-R_{2k}(S^{(2k)}(\lambda/2))\biggr)\biggr\|\nn
        &\leq R_{2k}\biggl(\exp(|\lambda|L\Lambda/2)\biggr) + R_{2k}\biggl(\exp(|\lambda|[2\cdot 5^{k-1}(L-1)+1]\Lambda/2)\biggr) \nn
        &\leq \frac{(|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp(|\lambda|L\Lambda/2)+ \frac{(|\lambda|[2\cdot 5^{k-1}(L-1)+1]\Lambda/2)^{2k+1}}{(2k+1)!}\exp(|\lambda|[2\cdot 5^{k-1}(L-1)+1]\Lambda/2)\nn
        &\leq 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp(\kappa|\lambda|L\Lambda/2).
    \end{align}
    Therefore, this gives us
    \begin{align} \label{2VD}
        \|V^{\dagger}\| \|D \| 
        &\leq \exp(|\lambda|L\Lambda/2)\cdot 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp(\kappa|\lambda|L\Lambda/2)\nn
        &=2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
    \end{align}
\end{proof}
\begin{lemma} \label{bound_A'}
Define $A$ as in Eq.~(\ref{A}), we can bound its value as
\begin{align}
 A\leq 4\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
\end{align}
\end{lemma}
\begin{proof}
    From the definition in Eq.~(\ref{A}), we use the triangle inequality to have
    \begin{align}
    A &:= \sum_{l \in \gamma}\sum_{h=1}^{L_{l}} \frac{|\lambda|^l}{2^{l}} |\beta_{h}^{(l)}|  \|H_{h}^{(l)}\|
    \leq \|V^{\dagger}D + DV^{\dagger} \| \leq 2 \|V^{\dagger}\| \|D \|.
    \end{align}
    By using Lemma \ref{V_D}, we have the bound 
    \begin{align}
        A \leq 4\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
    \end{align}
\end{proof}

\label{app:proofs}
\begin{comment}
\subsection{Proof of Lemma~\ref{2k+q order error}} \label{proof_of_lemma}
\begin{proof}
First, we have
\begin{equation} \label{U_h-U_h}
\begin{split}
    \langle U_h \rangle \langle U_h \rangle^{\dagger}
    &=(W+\langle \delta_h\rangle)(W+\langle \delta_h\rangle)^{\dagger}\\
    &=I+W(\langle \delta_h\rangle)^{\dagger}+\langle \delta_h\rangle W^{\dagger}+\langle \delta_h\rangle \langle \delta_h \rangle^{\dagger}.
\end{split}
\end{equation}
On the other hand, we consider the equation
\begin{equation}
    U_h=\langle U_h \rangle + d_h^{(\geq 2k+1)},
\end{equation}
where $d_h^{(\geq 2k+1)}$ is the difference between $U_h$ and $\langle U_h \rangle$.
Then we have
\begin{equation}
\begin{split}
    U_h U_h^{\dagger}
    &=(\langle U_h \rangle + d_h^{(\geq 2k+1)})(\langle U_h \rangle + d_h^{(\geq 2k+1)})^{\dagger}\\
    &= \langle U_h \rangle \langle U_h \rangle^{\dagger} + \langle U_h \rangle  (d_h^{(\geq 2k+1)})^{\dagger} + d_h^{(\geq 2k+1)} \langle U_h \rangle^{\dagger} +  d_h^{(\geq 2k+1)}(d_h^{(\geq 2k+1)})^{\dagger},
\end{split}
\end{equation}
where its average can be written as
\begin{equation}
\langle U_h U_h^{\dagger} \rangle = \langle U_h \rangle  \langle U_h \rangle^{\dagger}+ \langle d_h^{(\geq 2k+1)} ({d_h^{(\geq 2k+1)}})^{\dagger} \rangle,
\end{equation}
and it can be further simplified into
\begin{equation} \label{U_h U_h}
    \langle U_h \rangle \langle U_h \rangle^{\dagger}=I-\langle d_h^{(\geq 2k+1)} (d_h^{(\geq 2k+1)})^{\dagger}\rangle.
\end{equation}
Then we substitute Eq.~(\ref{U_h U_h}) into Eq.~(\ref{U_h-U_h}) to give
\begin{equation} \label{V-delta}
 W\langle \delta_h \rangle^{\dagger} + \langle \delta_h \rangle W^{\dagger} + \langle \delta_h \rangle \langle \delta_h \rangle^{\dagger}     +\langle d_h^{(\geq 2k+1)}(d_h^{(\geq 2k+1)})^{\dagger} \rangle = 0.
\end{equation}
If we can find the proper unitary $\{U_h\}$ to average out the error terms at the $(2k+q-1)$th order and the terms of $\delta_h$ at the $(2k+q)$th order are all Hermitian, then we can set
\begin{equation}  \label{delta_h}
    \langle \delta_h \rangle = A(t/r)^{2k+q} +O((t/r)^{2k+q+1}),
\end{equation}
where $A$ is a Hermitian operator to be determined. Then we replace Eq.~\eqref{delta_h} into Eq.~\eqref{V-delta} to give
\begin{equation}
    2A(t/r)^{2k+q}+O((t/r)^{2k+q+1})=0,
\end{equation}
provided $2k \ge q$.
We require the equation to hold for any $t \in \mathbb{R},r\in \mathbb{N^{+}}$ and $t/r \ll 1$, and, therefore, $A$ should be a zero matrix, and this shows that the error at the $(2k+q)$th order is also canceled out simultaneously once we correct the error terms at the $(2k+q-1)$th order.

In conclusion, when we find a way to cancel out the terms at the order $2k+1,2k+3,..,4k+1$, the terms at the order $2k+2,2k+4,...,4k$ vanish simultaneously, and this leads to $\langle\delta_{h}\rangle=O(\lambda^{4k+2})$. 
\end{proof}
\end{comment}

\subsection{Lemmas for the remainder}
The following two lemmas are used in the proof of Lemma \ref{find a_4k+2} and \ref{find b_4k+2} \cite{childs2019faster}. We define for any $k \in \mathbb{N}^{+}$ and any analytic function $f:\mathbb{C} \to \mathbb{C}$ with $f(\lambda)=\sum_{j=0}^{\infty}a_{j}\lambda^{j}$, and then $R_{k}(f):=\sum_{j=k+1}^{\infty}a_{j}\lambda^{j}$ is the remainder of the Taylor series expansion of the function $f(\lambda)$ up to order $k$.
\begin{lemma} \label{R_k}
If $\lambda$ is a complex number and $H_{1}, H_{2}..., H_{L}$ are Hermitian operators, then
\begin{equation}
    \biggl\Vert R_{k}\biggl( \prod_{i=1}^{L} \exp(\lambda H_{i}) \biggr)\biggr\Vert \leq R_{k}\biggl( \exp\biggl(\sum_{i=1}^{L}|\lambda|\cdot \Vert H_{i}\Vert \biggr)\biggr).
\end{equation}
\end{lemma}
\begin{lemma} \label{R_k_bound}
If $\lambda$ is a complex number, then
\begin{equation}
    |R_{k}(\exp(\lambda))|\leq \frac{|\lambda|^{k+1}}{(k+1)!}\exp(|\lambda|).
\end{equation}
\end{lemma}

\begin{comment}
\subsection{Lemma~\ref{alpha_bound}}
\begin{lemma}  (the upper bound for the coefficient $A_{h}^{(2k,q-1)}$) \label{A_bound}
    We can bound $|A_{h}^{(2k,q-1)}|$ as
    \begin{equation}
        |A_{h}^{(2k,q-1)}|\leq ,
    \end{equation}
    where $N=2\cdot 5^{k-1}(L-1)+1$.
    Then we have the bound for $\Vert H_{(h_{q},q/2)}' \Vert$
    \begin{equation}
    \Vert H_{(h_{q},q/2)}' \Vert \leq q (N\Lambda)^{2k+q-1}.
    \end{equation}
\end{lemma} 
\end{comment}

\begin{comment}
\begin{lemma} (the upper bound for the coefficient $\alpha_{h}^{(2k,q-1)}$)\label{alpha_bound}
We can bound $|\alpha_{h}^{(2k,q-1)}|$ as
\begin{equation}
    |\alpha_{h}^{(2k,q-1)}|\leq q N^{2k+q-1},
\end{equation}
where $N=2\cdot 5^{k-1}(L-1)+1$.
Then we have the bound for $\Vert H_{(h_{q},q/2)}' \Vert$
\begin{equation}
\Vert H_{(h_{q},q/2)}' \Vert \leq q (N\Lambda)^{2k+q-1}.
\end{equation}
\end{lemma}

\begin{proof}
From Eq.~(\ref{S_{m_{(2k,q+2)}}}), we have the expansion of $S_{p}^{(2k,q)}$
\begin{equation}
    \begin{split}
    S_{p}^{(2k,q)} \quad  &\\
    =S_{p}^{(2k,1)} &+\frac{2^{q/2}}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl( \lambda^{2k+q'-1}H_{(h_{q'},q'/2)}'\biggr)\\
         &  +\frac{1}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl\{\sum_{l=1}^{q-q'+1} \lambda^{l} \mathcal{H}_{l} , \lambda^{2k+q'-1} H_{(h_{q'},q'/2)}'\biggr\}\\
         & +\frac{1}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl\{\sum_{l=q-q'+2}^{\infty} \lambda^{l} \mathcal{H}_{l} , \lambda^{2k+q'-1} H_{(h_{q'},q'/2)}'\biggr\}\\
    %
    &+ R_{4k+1}(S_{p}^{(2k,q)}).
    \end{split}
\end{equation}
where the error terms at the $(2k+q'-1)$th order for $q \in \{2,4,...,q\}$ are contributed from two parts: one is from the $(2k+q'-1)$th order in $S_{p}^{(2k,1)}$ and the other is from the cross terms of the product of $S_{p}^{(2k,1)}$ and those $(2k+q'-1)$th-order correction
\begin{equation}  \label{expand_S_{p}^{(2k,q)}}
   \frac{1}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl\{\sum_{l=1}^{q-q'+1} \lambda^{l} \mathcal{H}_{l} , \lambda^{2k+q'-1} H_{(h_{q'},q'/2)}'\biggr\}.
\end{equation}
When we expand each exponentials individually in $S_{2k}^{\sigma}$ for $\sigma \in \operatorname{Sym}(L)$ and average over it to obtain $S_{p}^{(2k,1)}$, because $|p_{k}|\leq 1$ and $|1-4p_{k}|\leq 1$, the number of the terms at the $(2k+q-1)$th order with the multiplying coefficients lesser than one is no more than $N^{2k+q-1}$. This implies that we can uniformly split each term at the $(2k+q-1)$th order to no more than $N^{2k+q-1}$ terms with the coefficients of each of these terms lesser than one, which indicates that the number of the elements in the set $\eta^{(2k+q-1)}$ can be no more than $N^{2k+q-1}$ as well. Next, considering those $(2k+q-1)$th-order error from the cross term in the product of $(2k+q'-1)$th correction and $S_{p}^{(2k,1)}$ for each $q'\in \{2,4,...,q-2\}$, because the number of terms at the $(q-q')$th order is no more than $N^{q-q'}$, in total, this contributes the $(2k+q-1)$th-order error with the number
\begin{equation}
N^{2k+1} N^{q-2}+N^{2k+3} N^{q-4}+\cdots + N^{2k+q-3} N^{2}.
\end{equation}
Therefore, we can bound $n_{q}$ as 
\begin{equation}
    n_{q}\leq N^{2k+1}N^{q-2} + N^{2k+3}N^{q-4}+...+N^{2k+q-3}N^{2}+N^{2k+q-1}=\frac{q}{2}N^{2k+q-1}.
\end{equation}
Then from the choosing criterion Eq.~\eqref{alpha__beta}, for each $j\in \{1,2,...,m_{i}^{(l)}\}$ and $i\in \gamma^{(2k,q)}$, we have the bound
\begin{equation}
    \biggl|\alpha_{(i,j)}^{(2k,q-1)}\biggr|=\frac{n_{q}}{m_{i}^{(l)}}\biggl|\frac{1}{(2k+q-1)!}-\beta_{(i,j)}^{(2k+q-1,2k,q)}\biggr| \leq 2n_{q}\leq q N^{2k+q-1}.
\end{equation}
Then we have the bound
\begin{equation}
    \Vert H_{(h_{q},q/2)}' \Vert=|\alpha_{h_{q}}^{(2k,q-1)}|\cdot \Vert H_{h_{q}}^{(2k+q-1)}\Vert \leq q (N\Lambda)^{2k+q-1}.
\end{equation}
\end{proof}
\end{comment}

\section{Appendix} \label{appendix}
\subsection{For the case of Trotter-Suzuki formula}
\begin{lemma} \label{V_D}
When we consider the $(2k)$th-order Trotter-Suzuki formula in Eq.~(\ref{S_V_D}), we have the bound
\begin{align}
    \| V^{\dagger}(\lambda/2) \| \|D(\lambda/2)\| \leq 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
\end{align}
\end{lemma}
\begin{proof}
     If we consider $S^{(2k)}(\lambda/2)$ as the $(2k)$th-order Trotter-Suzuki formula, we have
    \begin{align}
        \|D\|
        &=\biggl\| R_{2k}\biggl(\exp(\lambda \sum_{i=1}^{L}H_{i}/2)-R_{2k}(S^{(2k)}(\lambda/2))\biggr)\biggr\|\nn
        &\leq R_{2k}\biggl(\exp(|\lambda|L\Lambda/2)\biggr) + R_{2k}\biggl(\exp(|\lambda|[2\cdot 5^{k-1}(L-1)+1]\Lambda/2)\biggr) \nn
        &\leq \frac{(|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp(|\lambda|L\Lambda/2)+ \frac{(|\lambda|[2\cdot 5^{k-1}(L-1)+1]\Lambda/2)^{2k+1}}{(2k+1)!}\exp(|\lambda|[2\cdot 5^{k-1}(L-1)+1]\Lambda/2)\nn
        &\leq 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp(\kappa|\lambda|L\Lambda/2).
    \end{align}
    Therefore, this gives us
    \begin{align} \label{2VD}
        \|V^{\dagger}\| \|D \| 
        &\leq \exp(|\lambda|L\Lambda/2)\cdot 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp(\kappa|\lambda|L\Lambda/2)\nn
        &=2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
    \end{align}
\end{proof}
\begin{lemma} \label{bound_A'}
Define $A$ as in Eq.~(\ref{A}), we can bound its value as
\begin{align}
 A\leq 4\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
\end{align}
\end{lemma}
\begin{proof}
    From the definition in Eq.~(\ref{A}), we use the triangle inequality to have
    \begin{align}
    A &:= \sum_{l \in \gamma}\sum_{h=1}^{L_{l}} \frac{|\lambda|^l}{2^{l}} |\beta_{h}^{(l)}|  \|H_{h}^{(l)}\|
    \leq \|V^{\dagger}D + DV^{\dagger} \| \leq 2 \|V^{\dagger}\| \|D \|.
    \end{align}
    By using Lemma \ref{V_D}, we have the bound 
    \begin{align}
        A \leq 4\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
    \end{align}
\end{proof}

\label{app:proofs}
\begin{comment}
\subsection{Proof of Lemma~\ref{2k+q order error}} \label{proof_of_lemma}
\begin{proof}
First, we have
\begin{equation} \label{U_h-U_h}
\begin{split}
    \langle U_h \rangle \langle U_h \rangle^{\dagger}
    &=(W+\langle \delta_h\rangle)(W+\langle \delta_h\rangle)^{\dagger}\\
    &=I+W(\langle \delta_h\rangle)^{\dagger}+\langle \delta_h\rangle W^{\dagger}+\langle \delta_h\rangle \langle \delta_h \rangle^{\dagger}.
\end{split}
\end{equation}
On the other hand, we consider the equation
\begin{equation}
    U_h=\langle U_h \rangle + d_h^{(\geq 2k+1)},
\end{equation}
where $d_h^{(\geq 2k+1)}$ is the difference between $U_h$ and $\langle U_h \rangle$.
Then we have
\begin{equation}
\begin{split}
    U_h U_h^{\dagger}
    &=(\langle U_h \rangle + d_h^{(\geq 2k+1)})(\langle U_h \rangle + d_h^{(\geq 2k+1)})^{\dagger}\\
    &= \langle U_h \rangle \langle U_h \rangle^{\dagger} + \langle U_h \rangle  (d_h^{(\geq 2k+1)})^{\dagger} + d_h^{(\geq 2k+1)} \langle U_h \rangle^{\dagger} +  d_h^{(\geq 2k+1)}(d_h^{(\geq 2k+1)})^{\dagger},
\end{split}
\end{equation}
where its average can be written as
\begin{equation}
\langle U_h U_h^{\dagger} \rangle = \langle U_h \rangle  \langle U_h \rangle^{\dagger}+ \langle d_h^{(\geq 2k+1)} ({d_h^{(\geq 2k+1)}})^{\dagger} \rangle,
\end{equation}
and it can be further simplified into
\begin{equation} \label{U_h U_h}
    \langle U_h \rangle \langle U_h \rangle^{\dagger}=I-\langle d_h^{(\geq 2k+1)} (d_h^{(\geq 2k+1)})^{\dagger}\rangle.
\end{equation}
Then we substitute Eq.~(\ref{U_h U_h}) into Eq.~(\ref{U_h-U_h}) to give
\begin{equation} \label{V-delta}
 W\langle \delta_h \rangle^{\dagger} + \langle \delta_h \rangle W^{\dagger} + \langle \delta_h \rangle \langle \delta_h \rangle^{\dagger}     +\langle d_h^{(\geq 2k+1)}(d_h^{(\geq 2k+1)})^{\dagger} \rangle = 0.
\end{equation}
If we can find the proper unitary $\{U_h\}$ to average out the error terms at the $(2k+q-1)$th order and the terms of $\delta_h$ at the $(2k+q)$th order are all Hermitian, then we can set
\begin{equation}  \label{delta_h}
    \langle \delta_h \rangle = A(t/r)^{2k+q} +O((t/r)^{2k+q+1}),
\end{equation}
where $A$ is a Hermitian operator to be determined. Then we replace Eq.~\eqref{delta_h} into Eq.~\eqref{V-delta} to give
\begin{equation}
    2A(t/r)^{2k+q}+O((t/r)^{2k+q+1})=0,
\end{equation}
provided $2k \ge q$.
We require the equation to hold for any $t \in \mathbb{R},r\in \mathbb{N^{+}}$ and $t/r \ll 1$, and, therefore, $A$ should be a zero matrix, and this shows that the error at the $(2k+q)$th order is also canceled out simultaneously once we correct the error terms at the $(2k+q-1)$th order.

In conclusion, when we find a way to cancel out the terms at the order $2k+1,2k+3,..,4k+1$, the terms at the order $2k+2,2k+4,...,4k$ vanish simultaneously, and this leads to $\langle\delta_{h}\rangle=O(\lambda^{4k+2})$. 
\end{proof}
\end{comment}

\subsection{Lemmas for the remainder}
The following two lemmas are used in the proof of Lemma \ref{find a_4k+2} and \ref{find b_4k+2} \cite{childs2019faster}. We define for any $k \in \mathbb{N}^{+}$ and any analytic function $f:\mathbb{C} \to \mathbb{C}$ with $f(\lambda)=\sum_{j=0}^{\infty}a_{j}\lambda^{j}$, and then $R_{k}(f):=\sum_{j=k+1}^{\infty}a_{j}\lambda^{j}$ is the remainder of the Taylor series expansion of the function $f(\lambda)$ up to order $k$.
\begin{lemma} \label{R_k}
If $\lambda$ is a complex number and $H_{1}, H_{2}..., H_{L}$ are Hermitian operators, then
\begin{equation}
    \biggl\Vert R_{k}\biggl( \prod_{i=1}^{L} \exp(\lambda H_{i}) \biggr)\biggr\Vert \leq R_{k}\biggl( \exp\biggl(\sum_{i=1}^{L}|\lambda|\cdot \Vert H_{i}\Vert \biggr)\biggr).
\end{equation}
\end{lemma}
\begin{lemma} \label{R_k_bound}
If $\lambda$ is a complex number, then
\begin{equation}
    |R_{k}(\exp(\lambda))|\leq \frac{|\lambda|^{k+1}}{(k+1)!}\exp(|\lambda|).
\end{equation}
\end{lemma}

\begin{comment}
\subsection{Lemma~\ref{alpha_bound}}
\begin{lemma}  (the upper bound for the coefficient $A_{h}^{(2k,q-1)}$) \label{A_bound}
    We can bound $|A_{h}^{(2k,q-1)}|$ as
    \begin{equation}
        |A_{h}^{(2k,q-1)}|\leq ,
    \end{equation}
    where $N=2\cdot 5^{k-1}(L-1)+1$.
    Then we have the bound for $\Vert H_{(h_{q},q/2)}' \Vert$
    \begin{equation}
    \Vert H_{(h_{q},q/2)}' \Vert \leq q (N\Lambda)^{2k+q-1}.
    \end{equation}
\end{lemma} 
\end{comment}

\begin{comment}
\begin{lemma} (the upper bound for the coefficient $\alpha_{h}^{(2k,q-1)}$)\label{alpha_bound}
We can bound $|\alpha_{h}^{(2k,q-1)}|$ as
\begin{equation}
    |\alpha_{h}^{(2k,q-1)}|\leq q N^{2k+q-1},
\end{equation}
where $N=2\cdot 5^{k-1}(L-1)+1$.
Then we have the bound for $\Vert H_{(h_{q},q/2)}' \Vert$
\begin{equation}
\Vert H_{(h_{q},q/2)}' \Vert \leq q (N\Lambda)^{2k+q-1}.
\end{equation}
\end{lemma}

\begin{proof}
From Eq.~(\ref{S_{m_{(2k,q+2)}}}), we have the expansion of $S_{p}^{(2k,q)}$
\begin{equation}
    \begin{split}
    S_{p}^{(2k,q)} \quad  &\\
    =S_{p}^{(2k,1)} &+\frac{2^{q/2}}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl( \lambda^{2k+q'-1}H_{(h_{q'},q'/2)}'\biggr)\\
         &  +\frac{1}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl\{\sum_{l=1}^{q-q'+1} \lambda^{l} \mathcal{H}_{l} , \lambda^{2k+q'-1} H_{(h_{q'},q'/2)}'\biggr\}\\
         & +\frac{1}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl\{\sum_{l=q-q'+2}^{\infty} \lambda^{l} \mathcal{H}_{l} , \lambda^{2k+q'-1} H_{(h_{q'},q'/2)}'\biggr\}\\
    %
    &+ R_{4k+1}(S_{p}^{(2k,q)}).
    \end{split}
\end{equation}
where the error terms at the $(2k+q'-1)$th order for $q \in \{2,4,...,q\}$ are contributed from two parts: one is from the $(2k+q'-1)$th order in $S_{p}^{(2k,1)}$ and the other is from the cross terms of the product of $S_{p}^{(2k,1)}$ and those $(2k+q'-1)$th-order correction
\begin{equation}  \label{expand_S_{p}^{(2k,q)}}
   \frac{1}{N_{q}}\sum_{q' \in\{2,4,...,q\}}\sum_{h_{q'}} \biggl\{\sum_{l=1}^{q-q'+1} \lambda^{l} \mathcal{H}_{l} , \lambda^{2k+q'-1} H_{(h_{q'},q'/2)}'\biggr\}.
\end{equation}
When we expand each exponentials individually in $S_{2k}^{\sigma}$ for $\sigma \in \operatorname{Sym}(L)$ and average over it to obtain $S_{p}^{(2k,1)}$, because $|p_{k}|\leq 1$ and $|1-4p_{k}|\leq 1$, the number of the terms at the $(2k+q-1)$th order with the multiplying coefficients lesser than one is no more than $N^{2k+q-1}$. This implies that we can uniformly split each term at the $(2k+q-1)$th order to no more than $N^{2k+q-1}$ terms with the coefficients of each of these terms lesser than one, which indicates that the number of the elements in the set $\eta^{(2k+q-1)}$ can be no more than $N^{2k+q-1}$ as well. Next, considering those $(2k+q-1)$th-order error from the cross term in the product of $(2k+q'-1)$th correction and $S_{p}^{(2k,1)}$ for each $q'\in \{2,4,...,q-2\}$, because the number of terms at the $(q-q')$th order is no more than $N^{q-q'}$, in total, this contributes the $(2k+q-1)$th-order error with the number
\begin{equation}
N^{2k+1} N^{q-2}+N^{2k+3} N^{q-4}+\cdots + N^{2k+q-3} N^{2}.
\end{equation}
Therefore, we can bound $n_{q}$ as 
\begin{equation}
    n_{q}\leq N^{2k+1}N^{q-2} + N^{2k+3}N^{q-4}+...+N^{2k+q-3}N^{2}+N^{2k+q-1}=\frac{q}{2}N^{2k+q-1}.
\end{equation}
Then from the choosing criterion Eq.~\eqref{alpha__beta}, for each $j\in \{1,2,...,m_{i}^{(l)}\}$ and $i\in \gamma^{(2k,q)}$, we have the bound
\begin{equation}
    \biggl|\alpha_{(i,j)}^{(2k,q-1)}\biggr|=\frac{n_{q}}{m_{i}^{(l)}}\biggl|\frac{1}{(2k+q-1)!}-\beta_{(i,j)}^{(2k+q-1,2k,q)}\biggr| \leq 2n_{q}\leq q N^{2k+q-1}.
\end{equation}
Then we have the bound
\begin{equation}
    \Vert H_{(h_{q},q/2)}' \Vert=|\alpha_{h_{q}}^{(2k,q-1)}|\cdot \Vert H_{h_{q}}^{(2k+q-1)}\Vert \leq q (N\Lambda)^{2k+q-1}.
\end{equation}
\end{proof}
\end{comment}

\begin{comment}
where 
\begin{align}
     \| V^{\dagger}(\lambda/2) \| \|D(\lambda/2)\| \leq 2\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2),
\end{align}
and 
\begin{align}
    A\leq 4\frac{(\kappa|\lambda|L\Lambda/2)^{2k+1}}{(2k+1)!}\exp([\kappa+1]|\lambda|L\Lambda/2).
\end{align}

Now we use the triangle bound to have
\begin{align}   \label{VS}
    &\biggl\Vert V^{\dagger} \sum_{l\in \gamma}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
        \cdot U_{h}^{(l)}-I \biggr\Vert \\
    &\le \biggl\Vert \sum_{\ell=4k+2}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}' \biggl\Vert+ \biggl\Vert \left( \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}' \right) \left(  \sum_{l\in \gamma} \lambda^{l} \mathcal{H}_{l}'\right) \biggl\Vert  \label{VS_2}  \\
    & \quad \quad +\biggl\Vert \biggl(I+ \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}'\biggr) \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\sum_{i=2}^{\infty}\frac{1}{i!}(\alpha_{h,l} H_{h}^{(l)})^{i} \biggl\Vert  \label{VS_3}. 
\end{align}
Next, we bound each norms in Eq.~(\ref{VS_2}) and Eq.~(\ref{VS_3}) individually.
By using the Lemma 3 in \cite{childs2019faster}, the $s$th-order error of $S_{p}^{(2k)}-V$ is given as
%{\color{red}Incomplete here?}
   \begin{equation}
        \begin{split}
    &\left\{
    \begin{array}{rcl}
    0       &0\leq s\leq 2k,\\
    \frac{(\kappa |\lambda|\Lambda)^{s}}{(s-2)!}L^{s-1} &s>2k,
    \end{array} \right.
        \end{split}
    \end{equation}
    where $\kappa:=2\cdot 5^{k-1}$.
First, starting from Eq.~(\ref{H'}), we have
\begin{align} \label{lambda_bound}
    \biggl\Vert \sum_{l=2k+1}^{\infty} \lambda^{l} \mathcal{H}_{l}' \biggr\Vert
    %=\biggl \Vert V^{\dagger}S_{p}^{(2k)}-I \biggr \Vert
    &=\biggl \Vert V^{\dagger}\biggl( S_{p}^{(2k)}-V\biggr) \biggr \Vert \\
    &\leq  \exp(|\lambda|L\Lambda)\cdot\sum_{s=2k+1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s}L^{s-1}}{(s-2)!} \\
    &=  \exp(|\lambda|L\Lambda)\cdot\sum_{s'=2k-1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s'+2}L^{s'+1}}{s'!},
\end{align}
where we set $s'=s-2$.
Then we can have the bound by using Lemma.~\ref{R_k_bound}
\begin{align} 
    \biggl\Vert \sum_{l=2k+1}^{\infty} \lambda^{l} \mathcal{H}_{l}' \biggr\Vert
    &\leq  \exp(|\lambda|L\Lambda)\cdot (\kappa |\lambda|\Lambda)^{2}L \cdot R_{2k-2}\biggl(\exp(\kappa |\lambda|L\Lambda)\biggr)\\
    &\leq  \exp(|\lambda|L\Lambda)\cdot (\kappa |\lambda|\Lambda)^{2}L \cdot \frac{(\kappa |\lambda|L\Lambda)^{2k-1}}{(2k-1)!}\exp(\kappa |\lambda|L\Lambda)\\
    &= \frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1) |\lambda|L\Lambda]. \label{l_2k+1_infty}
\end{align}
Therefore, we can bound the first norm in Eq.~(\ref{VS_2}) as
\begin{equation}
\begin{split}
\biggl\Vert \sum_{l=4k+2}^{\infty} \lambda^{l} \mathcal{H}_{l}' \biggr\Vert
%=\biggl \Vert R_{4k+1}\biggl(V^{\dagger}S_{p}^{(2k)}-I\biggr) \biggr \Vert
&=\biggl \Vert R_{4k+1}\biggl(V^{\dagger}\biggl( S_{p}^{(2k)}-V\biggr)\biggr) \biggr \Vert \\
&\leq R_{4k+1}\biggl(\frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1) |\lambda|L\Lambda ]\biggr) \\
&\leq \frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}R_{2k}\biggl(\exp[(\kappa+1) |\lambda|L\Lambda ]\biggr).
\end{split}
\end{equation}
Then we have the bound by using Lemma.~\ref{R_k_bound}
\begin{equation}
\begin{split}
\biggl\Vert \sum_{l=4k+2}^{\infty} \lambda^{l} \mathcal{H}_{l}' \biggr\Vert
&\leq \frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\sum_{i=2k+1}^{\infty}\frac{[(\kappa+1) |\lambda|L\Lambda )]^{i}}{i!}\\
& \leq \frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!} \frac{[(\kappa+1) |\lambda|L\Lambda )]^{2k+1}}{(2k+1)!}\exp[(\kappa+1) |\lambda|L\Lambda )] \\
&= \frac{[\kappa(\kappa+1)]^{2k+1}(|\lambda|\Lambda)^{4k+2}L^{4k+1}}{(2k-1)!(2k+1)!}\exp[(\kappa+1) |\lambda|L\Lambda )].
\end{split}
\end{equation}
Therefore, we bound the norm as 
\begin{align}
    \biggl \Vert R_{4k+1}\biggl(V^{\dagger}\biggl( S_{p}^{(2k)}-V\biggr)\biggr) \biggr \Vert 
    &\leq \sum_{i=2k+1}^{\infty}\frac{(|\lambda|L\Lambda)^{i}}{i!}\cdot \sum_{s=2k+1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s}}{(s-2)!}L^{s-1}\\
    &=\sum_{i=2k+1}^{\infty}\frac{(|\lambda|L\Lambda)^{i}}{i!}\cdot\sum_{s'=2k-1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s'+2}L^{s'+1}}{s'!},
\end{align}
where we set $s'=s-2$. Hence, we can have the bound 
\begin{align}
    \biggl\Vert \sum_{l=4k+2}^{\infty} \lambda^{l} \mathcal{H}_{l}' \biggr\Vert 
    &\leq \sum_{i=2k+1}^{\infty}\frac{(|\lambda|L\Lambda)^{i}}{i!}\cdot\sum_{s'=2k-1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s'+2}L^{s'+1}}{s'!} \\
    &= (\kappa |\lambda|\Lambda)^{2}L \sum_{i=2k+1}^{\infty}\frac{(|\lambda|L\Lambda)^{i}}{i!}\cdot\sum_{s'=2k-1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s'}L^{s'}}{s'!} \\
    &\leq (\kappa |\lambda|\Lambda)^{2}L\cdot \frac{(|\lambda|L\Lambda)^{2k+1}}{(2k+1
    )!}\exp(|\lambda|L\Lambda)\cdot \frac{(\kappa |\lambda|L\Lambda)^{2k-1}}{(2k-1)!}\exp(\kappa |\lambda|L\Lambda)\\
    &= \frac{\kappa^{2k+1} (|\lambda|\Lambda)^{4k+2}L^{4k+1}}{(2k-1)!(2k+1)!}\exp\biggl(|\lambda|L\Lambda(\kappa+1)\biggr),
\end{align}
where we use Lemma.~\ref{R_k_bound} in the last inequality.
%Then for $I-V^{\dagger}S_{p}^{(2k)}$
%\begin{align}
%    \biggl\Vert \sum_{\ell=4k+2}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}' \biggl\Vert 
%    \le \sum_{s=4k+2}^{\infty}\frac{(\kappa \Lambda |\lambda|)^{s}L^{s-1}}{(s-2)!}
%    \le \frac{(\kappa \Lambda |\lambda|)^{4k+2}L^{4k+2}}{(4k+1)!}
%\end{align}
%{\color{red}This can't be right.  It has a spurious extra $L^{4k+2}$, and it only has the leading order term.}
For the second norm, similarly, we have
\begin{align}
    \biggl\Vert \sum_{l=2k+1}^{\infty} \lambda^{l} \mathcal{H}_{l}' \biggr\Vert=\biggl \Vert \biggl(V^{\dagger}S_{p}^{(2k)}-I\biggr) \biggr \Vert
    &=\biggl \Vert \biggl(V^{\dagger}\biggl( S_{p}^{(2k)}-V\biggr)\biggr) \biggr \Vert \\
    &\leq  \exp(|\lambda|L\Lambda)\cdot\sum_{s'=2k-1}^{\infty}\frac{(\kappa |\lambda|\Lambda)^{s'+2}L^{s'+1}}{s'!} \\
    &\leq  \exp(|\lambda|L\Lambda)\cdot (\kappa |\lambda|\Lambda)^{2}L \frac{(\kappa |\lambda|L\Lambda)^{2k-1}}{(2k-1)!}\exp(\kappa |\lambda|L\Lambda)\\
    &= \frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp((\kappa+1) |\lambda|L\Lambda)
\end{align}
Subsequently, by using the bound in Eq.~(\ref{l_2k+1_infty}) and some norm properties, we can bound the second norm in Eq.~(\ref{VS_2}) as
\begin{equation}
\begin{split}
    \left\| \left( \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}' \right) \left(  \sum_{l\in \gamma} \lambda^{l} \mathcal{H}_{l}'\right)\right\| 
    &\le \left\| \left( \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}' \right) \right\|\cdot \left\| \left(  \sum_{l\in \gamma} \lambda^{l} \mathcal{H}_{l}'\right)\right\| \\
    &\le \left[\frac{(\kappa  |\lambda| \Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1)  |\lambda|L\Lambda]\right]^2\\
    &\le \frac{(\kappa |\lambda|\Lambda )^{4k+2}L^{4k}}{((2k-1)!)^{2}}\exp[2(\kappa+1)  |\lambda|L\Lambda].
\end{split}
\end{equation}
At last, for the third norm in Eq.~(\ref{VS_3}), we have
\begin{align} \label{I+H}
    &\biggl\Vert \biggl(I+ \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}'\biggr)   \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\sum_{i=2}^{\infty}\frac{1}{i!}(\alpha_{h,l} H_{h}^{(l)})^{i} \biggl\Vert \\
    &\leq \biggl(1+ \biggl\Vert  \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}'\biggr \Vert \biggr) \cdot \biggl\Vert \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\sum_{i=2}^{\infty}\frac{1}{i!}(\alpha_{h,l} H_{h}^{(l)})^{i} \biggl\Vert. \label{I+H2}
\end{align}
Among Eq.~(\ref{I+H2}), we use some standard properties of norms, the definition in Eq.~(\ref{alpha}), Eq.~(\ref{A'_epsilon}), and Eq.~(\ref{A'}) to have
\begin{align}
    \biggl\Vert \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\sum_{i=2}^{\infty}\frac{1}{i!}(\alpha_{h,l} H_{h}^{(l)})^{i} \biggl\Vert 
    &=\biggl\Vert \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}| \alpha_{h,l}}{A}\sum_{i=2}^{\infty}\frac{1}{i!}\alpha_{h,l}^{i-1} {H_{h}^{(l)}}^{i} \biggl\Vert \\
    &=\biggl\Vert \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}(-\lambda^{l}\beta_{h}^{(l)})\sum_{i=2}^{\infty}\frac{1}{i!}\alpha_{h,l}^{i-1} {H_{h}^{(l)}}^{i} \biggl\Vert \\
    &\leq \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}|\lambda|^{l}|\beta_{h}^{(l)}|\sum_{i=2}^{\infty}\frac{1}{i!}\frac{(A)^{i-1}}{{\Vert H_{h}^{(l)}\Vert}^{i-1}} \Vert{H_{h}^{(l)}}\Vert^{i} \\
    &\leq \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}|\lambda|^{l}|\beta_{h}^{(l)}|\Vert{H_{h}^{(l)}}\Vert\sum_{i=2}^{\infty} \frac{(A)^{i-1}}{i!}\\
    &\leq \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}|\epsilon_{h,l}|\sum_{i=2}^{\infty} \frac{(A)^{i-1}}{i!}\\
    &=\sum_{i=2}^{\infty} \frac{(A)^{i}}{i!}\\
    &\leq \frac{A^{2}}{2}\exp(A),
\end{align}
where we use Lemma.~\ref{R_k_bound} in the last equality.
Therefore, we can bound the third norm as
\begin{align}
     &\biggl\Vert \biggl(I+ \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}'\biggr)   \sum_{l\in \gamma}\sum_{h=1}^{L_{l}}\frac {|\epsilon_{h,l}|}{A}\sum_{i=2}^{\infty}\frac{1}{i!}(\alpha_{h,l} H_{h}^{(l)})^{i} \biggl\Vert \\
     &\leq \biggl(1+ \biggl\Vert  \sum_{\ell=2k+1}^{\infty} \lambda^{\ell} \mathcal{H}_{\ell}'\biggr \Vert \biggr)\frac{A^{2}}{2}\exp(A)\\
     &\leq \biggl(1+\frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1) |\lambda|L\Lambda]\biggr)\frac{A^{2}}{2}\exp(A).
\end{align}
%{\color{red}There are a lot of missing steps here.}
%\begin{align}
%\left\|\sum_{l\in \gamma}\sum_{h=1}^{L_{l}} \lambda^l\beta_i^{(l)} \alpha_{h,l} (H_{h}^{(l)})^2\right\| &\le
%\sum_{l\in \gamma}\sum_{h=1}^{L_{l}} \lambda^l|\beta_i^{(l)}| \times \| H_{h}^{(l)}\| A \le A^2 .
%\end{align}
As a result, we have
\begin{equation}
\begin{split}
    \left\| V^{\dagger} \sum_{l\in \gamma}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
        \cdot U_{h}^{(l)}-I\right\| 
        &\le \frac{[\kappa(\kappa+1)]^{2k+1}(|\lambda|\Lambda)^{4k+2}L^{4k+1}}{(2k-1)!(2k+1)!}\exp[(\kappa+1) |\lambda|L\Lambda )]\\
        &\quad +  \frac{(\kappa |\lambda|\Lambda )^{4k+2}L^{4k}}{((2k-1)!)^{2}}\exp[2(\kappa+1)  |\lambda|L\Lambda] \\
        &\quad + \biggl(1+\frac{(\kappa |\lambda|L\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1) |\lambda|L\Lambda]\biggr)\frac{A^{2}}{2}\exp(|A|).
\end{split}
\end{equation}
%{\color{red}Why the factor of 2?  Wouldn't it be 1.5?}
In turn that implies
\begin{equation}
\begin{split}
    \biggl\| &V(\lambda) - \sum_{l=2k+1}^{4k+2}\sum_{h=1}^{L_{l}} p_{h,l} S_{p}^{(2k)}
        \cdot U_{h}^{(l)}\biggr\| \\
        &\le \exp(|\lambda|L\Lambda)\cdot \biggl[\frac{[\kappa(\kappa+1)]^{2k+1}(|\lambda|\Lambda)^{4k+2}L^{4k+1}}{(2k-1)!(2k+1)!}\exp[(\kappa+1) |\lambda|L\Lambda )]\\
        &\quad \quad \quad \quad \quad \quad \quad \quad +  \frac{(\kappa |\lambda|\Lambda )^{4k+2}L^{4k}}{((2k-1)!)^{2}}\exp[2(\kappa+1)  |\lambda|L\Lambda ] \\
        &\quad \quad \quad \quad \quad \quad \quad \quad + \biggl(1+\frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1) |\lambda|L\Lambda]\biggr)\frac{A^{2}}{2}\exp(A) \biggr]
\end{split}
\end{equation}
with 
    \begin{align}
        A\leq \frac{(\kappa |\lambda|\Lambda)^{2k+1}L^{2k}}{(2k-1)!}\exp[(\kappa+1) |\lambda|\Lambda L ].
    \end{align}
\end{comment}
